Finite-Sample Analysis of Policy Evaluation for Robust Average Reward Reinforcement Learning

We present the first finite-sample analysis of policy evaluation in robust average-reward Markov Decision Processes (MDPs). Prior work in this setting have established only asymptotic convergence guarantees, leaving open the question of sample complexity. In this work, we address this gap by showing that the robust Bellman operator is a contraction under a carefully constructed semi-norm, and developing a stochastic approximation framework with controlled bias. Our approach builds upon Multi-Level Monte Carlo (MLMC) techniques to estimate the robust Bellman operator efficiently. To overcome the infinite expected sample complexity inherent in standard MLMC, we introduce a truncation mechanism based on a geometric distribution, ensuring a finite expected sample complexity while maintaining a small bias that decays exponentially with the truncation level. Our method achieves the order-optimal sample complexity of $\tilde{\mathcal{O}}(\epsilon^{-2})$ for robust policy evaluation and robust average reward estimation, marking a significant advancement in robust reinforcement learning theory.

==> Method.tex <==
\section{Proposed Approach}

\subsection{Estimators for $\sigma_{\cp^a_s}$}
\subsubsection{Linear Uncertainty Model: Contamination Uncertainty Set}
We directly follow \citep{wang2023model}'s method and utilize the transition to the subsequent state to construct our estimator:
\begin{align}\label{eq:12}
    \hat{\sigma}_{\cp^a_s}(V)\triangleq (1-\delta)\gamma V(s')+\delta\min_x V(x),
\end{align}
where $s'$ is a subsequent state sample after $(s,a)$. 
\subsubsection{Nonlinear Uncertainty Model}
For non-linear uncertainty sets such as KL divergence, TV divergence, Wasserstein distance and Chi-square, obtaining $\sigma_{\cp^a_s}$ from only accessing the nominal model is challenging. \citep{wang2023model} proposed a method using Multi-Level Monte Carlo (MLMC) approach for obtaining an unbiased estimator $\hat{\sigma}_{\cp^a_s}$ with bounded variance. However,  this approach requires performing $2^N$ samples whereas $N$ sampled from a geometric distribution $Geo(\Psi)$ with parameter $\Psi \in (0,0.5)$. As a result, the expected number of samples for obtaining a single $\hat{\sigma}_{\cp^a_s}$ is infinity. To cope with this problem, we modify the method in \citep{wang2023model} and propose a truncated MLMC approach.

For any $s,a$, we first generate $N$ according to a geometric distribution with parameter $\Psi\in(0,1)$. We then perform truncation via a predefined number $N_{\max}$ and set $N = \min\{N,N_{\max}\}$. Then, we take action $a$ at state $s$ for $2^{N+1}$ times, and observe $r(s,a)$ and the subsequent state $\{s_i'\}, i=1,...,2^{N+1}$. We divide these $2^{N+1}$ samples into two groups:  samples with odd indices, and samples with even indices. We then individually calculate the empirical distribution of $s'$ using the even-index samples, odd-index ones, all the samples, and the first sample:
$\hat{\kp}^{a,E}_{s,N+1}= \frac{1}{2^{N}}\sum_{i=1}^{2^{N}}\mathbbm{1}_{s_{2i}'},  
\quad\hat{\kp}^{a,O}_{s,N+1}= \frac{1}{2^{N}}\sum_{i=1}^{2^{N}}\mathbbm{1}_{s_{2i-1}'},$
$\hat{\kp}^{a}_{s,N+1}= \frac{1}{2^{N+1}}\sum_{i=1}^{2^{N+1}}\mathbbm{1}_{s_i'},\quad\hat{\kp}^{a,1}_{s,N+1}= \mathbbm{1}_{s_1'}.
$
Then, we use these estimated transition kernels as nominal kernels to construct four estimated uncertainty sets $\hat{\cp}^{a,E}_{s,N+1},\hat{\cp}^{a,O}_{s,N+1},\hat{\cp}^{a}_{s,N+1},\hat{\cp}^{a,1}_{s,N+1}$. The multi-level estimator is then defined as 
\begin{align}\label{eq:est1}
    \hat{\sigma}_{\cp^a_s}(V)\triangleq \sigma_{\hat{\cp}^{a,1}_{s,N+1}}(V)+\frac{\Delta_N(V)}{p_N},
\end{align}
where  $p_N=
\begin{cases}
(1 - \Psi)^{k-1} \Psi, & 1 \leq N < N_{\max} \\
(1 - \Psi)^{N_{\max} - 1}, & N = N_{\max}
\end{cases}$ and
\begin{align}
    \Delta_N(V)\triangleq \sigma_{\hat{\cp}^{a}_{s,N+1}}(V)-\frac{\sigma_{\hat{\cp}^{a,E}_{s,N+1}}(V)+\sigma_{\hat{\cp}^{a,O}_{s,N+1}}(V)}{2}.\nn
\end{align}



\begin{theorem}[Truncated MLMC: Exponential Bias Decay and Bounded Variance]
\label{thm:trunc-mlmc}
Let $\hat{\sigma}_{\cp^a_s}(V)$ be the multi-level Monte Carlo (MLMC) estimator for the robust Bellman operator $\sigma_{\cp^a_s}(V)$ under any of the following uncertainty sets:
\begin{enumerate}
  \item Total Variation (TV) distance,
  \item Kullback--Leibler (KL) divergence,
  \item $\chi^2$ distance,
  \item Wasserstein distance (with discrete state space).
\end{enumerate}
Suppose (as shown in \citep{wang2023model}) that the \emph{untruncated} estimator $\hat{\sigma}_{\cp^a_s}(V)$ is \textbf{unbiased},
\begin{equation}
  \mathbb{E}\bigl[\hat{\sigma}_{\cp^a_s}(V)\bigr]
  \;=\;
  \sigma_{\cp^a_s}(V),
\end{equation}
and has \textbf{uniformly bounded variance},
\begin{equation}
  \mathrm{Var}\!\bigl[\hat{\sigma}_{\cp^a_s}(V)\bigr]
  \;\le\;
  C_0\,\|V\|^2
  \quad\text{for some constant }C_0.
\end{equation}
Then the \emph{truncated} estimator $\hat{\sigma}_{\cp^a_s}^{(\mathrm{tr})}(V)$, which cuts off the MLMC level at $N_{\max}$, satisfies:

\begin{enumerate}
\item \textbf{(Exponential Bias Decay)} There exist constants $C_1>0$ and $\gamma>0$, not depending on $N_{\max}$, such that
\begin{equation}
  \bigl|\,
     \mathbb{E}\bigl[\hat{\sigma}_{\cp^a_s}^{(\mathrm{tr})}(V)\bigr]
     \;-\;
     \sigma_{\cp^a_s}(V)
  \bigr|
  \;\le\;
  C_1\,\|V\|\,
  e^{-\gamma\,N_{\max}}.
\end{equation}
\item \textbf{(Bounded Variance)} There is a constant $C_2>0$, also not depending on $N_{\max}$, such that
\begin{equation}
  \mathrm{Var}\!\bigl[\hat{\sigma}_{\cp^a_s}^{(\mathrm{tr})}(V)\bigr]
  \;\le\;
  C_2\,\|V\|^2.
\end{equation}
\end{enumerate}
Here $\|\cdot\|$ denotes a suitable norm of $V$ (e.g.\ a supremum norm), and the constants $C_1, C_2, \gamma$ may depend on model parameters such as $\delta$ (the size of the uncertainty set), but they do not grow with $N_{\max}$.
\end{theorem}

\begin{proof}

\textbf{Step~1: Definition of the truncated estimator.}

Let $N$ be the geometric random level used in \citep{wang2023model}, with
\begin{equation}
  \mathbb{P}(N=n)
  \;=\;
  \Psi\,(1-\Psi)^{\,n}, 
  \quad
  n=0,1,2,\dots.
\end{equation}
Define the \emph{truncated} random level 
\begin{equation}
  N' \;=\;\min\{N,\;N_{\max}\},
\end{equation}
having probability mass function
\begin{equation}
  \mathbb{P}(N' = n)
  \;=\;
  \begin{cases}
    \Psi\,(1-\Psi)^n,
    &0\le n<N_{\max},\\[6pt]
    \sum_{m=N_{\max}}^{\infty}\!\Psi\,(1-\Psi)^{m}
    \;=\;(1-\Psi)^{N_{\max}},
    &n=N_{\max}.
  \end{cases}
\end{equation}
Exactly as in \citep{wang2023model}, for each level $n$ we form empirical distributions (including odd/even subsets) from $2^{n+1}$ i.i.d.\ samples.  Let
\begin{equation}
  \Delta_n(V)
  \;=\;
  \sigma_{\hat{\cp}^{\,a}_{s,n+1}}(V)
  \;-\;
  \tfrac12\Bigl[
    \sigma_{\hat{\cp}^{\,a,O}_{s,n+1}}(V)
    \;+\;
    \sigma_{\hat{\cp}^{\,a,E}_{s,n+1}}(V)
  \Bigr].
\end{equation}
Then the truncated MLMC estimator is
\begin{equation}
  \hat{\sigma}_{\cp^a_s}^{(\mathrm{tr})}(V)
  \;=\;
  \sigma_{\hat{\cp}^{\,a,1}_{s,N'+1}}(V)
  \;+\;
  \frac{\Delta_{\,N'}(V)}{p'(N')},
\end{equation}
where $p'(N')=\mathbb{P}(N'=N')$.  

\medskip

\textbf{Step~2: Exponential bias bound.}

From \citep{wang2023model}, we know that the \emph{untruncated} MLMC estimator $\hat{\sigma}_{\cp^a_s}(V)$ is unbiased:
\begin{equation}
  \mathbb{E}\!\bigl[\hat{\sigma}_{\cp^a_s}(V)\bigr]
  \;=\;
  \sigma_{\cp^a_s}(V).
\end{equation}
In particular, its expectation can be written (in a telescoping form) as 
\begin{equation}
  \mathbb{E}\!\bigl[\hat{\sigma}_{\cp^a_s}(V)\bigr]
  \;=\;
  \mathbb{E}\!\bigl[\sigma_{\hat{\cp}^{\,a,1}_{s,1}}(V)\bigr]
  \;+\;
  \sum_{n=0}^{\infty}\,\mathbb{E}\!\bigl[\Delta_n(V)\bigr].
\end{equation}
In the \emph{truncated} version, we instead cut off all levels $n > N_{\max}$, so
\begin{equation}
  \mathbb{E}\!\bigl[\hat{\sigma}_{\cp^a_s}^{(\mathrm{tr})}(V)\bigr]
  \;=\;
  \mathbb{E}\!\bigl[\sigma_{\hat{\cp}^{\,a,1}_{s,1}}(V)\bigr]
  \;+\;
  \sum_{n=0}^{\,N_{\max}}\,\mathbb{E}\!\bigl[\Delta_n(V)\bigr].
\end{equation}
Hence the bias arises exactly from the \emph{omitted} terms $n>N_{\max}$:
\begin{equation}
  \sigma_{\cp^a_s}(V)
  \;-\;
  \mathbb{E}\!\bigl[\hat{\sigma}_{\cp^a_s}^{(\mathrm{tr})}(V)\bigr]
  \;=\;
  \sum_{n=N_{\max}+1}^{\infty}\,\mathbb{E}\!\bigl[\Delta_n(V)\bigr].
\end{equation}

\noindent
\emph{Why does $\mathbb{E}[\Delta_n(V)]$ shrink exponentially?} 

\smallskip
\begin{itemize}
\item 
By construction,
\begin{equation}
  \Delta_n(V)
  \;=\;
  \sigma_{\hat{\cp}^{a}_{s,n+1}}(V)
  \;-\;\tfrac12\Bigl[
     \sigma_{\hat{\cp}^{a,O}_{s,n+1}}(V)
     \;+\;
     \sigma_{\hat{\cp}^{a,E}_{s,n+1}}(V)
  \Bigr],
\end{equation}
where $\hat{\cp}^{a}_{s,n+1}$ is the empirical distribution from $2^{n+1}$ i.i.d.\ samples, and $\hat{\cp}^{a,O}_{s,n+1},\hat{\cp}^{a,E}_{s,n+1}$ each come from half of those samples.

\item
All four divergences/distances (TV, KL, $\chi^2$, Wasserstein with a discrete state space) give a robust operator $\sigma_{p}(V)$ that is \emph{continuous} (often Lipschitz) in $p$.  Hence, if $p$ is close to the nominal $\cp^{a}_{s}$, we have 
\[
  \bigl|\sigma_{p}(V)-\sigma_{\cp^a_s}(V)\bigr|
  \;\le\;
  \mathrm{const}\,\|V\|
  \,\|p - \cp^a_s\|_1
  \quad(\text{or a similar local bound}).
\]
\item
By Hoeffding‐type binomial concentration, the empirical distributions $\hat{\cp}^{a}_{s,n+1}$ converge to $\cp^a_s$ at rate $\mathrm{O}(2^{-\,n/2})$ in expectation.  Thus
\[
  \mathbb{E}\Bigl[\bigl\lVert
     \hat{\cp}^{a}_{s,n+1}
     -\cp^a_s
  \bigr\rVert_1\Bigr]
  \;=\;
  \mathrm{O}\bigl(2^{-\,n/2}\bigr).
\]
\item
Consequently,
\[
  \bigl|\mathbb{E}[\sigma_{\hat{\cp}^{a}_{s,n+1}}(V)-\sigma_{\cp^a_s}(V)]\bigr|
  \;=\;
  \mathrm{O}\bigl(2^{-\,n/2}\bigr),
\]
and likewise for $\hat{\cp}^{a,O}_{s,n+1},\hat{\cp}^{a,E}_{s,n+1}$.  Therefore,
\[
  \mathbb{E}[|\Delta_n(V)|]
  \;\;=\;
  \mathrm{O}\bigl(2^{-\,n/2}\bigr).
\]
\end{itemize}

\noindent
Hence we obtain a \emph{geometric} tail for the omitted terms:
\begin{equation}
  \sum_{n=N_{\max}+1}^{\infty}\!\bigl|\mathbb{E}[\Delta_n(V)]\bigr|
  \;\;\le\;
  \mathrm{const}\,\|V\|
  \sum_{n=N_{\max}+1}^{\infty}2^{-\,n/2}
  \;\;=\;
  C_1\,\|V\|\;e^{-\gamma\,N_{\max}},
\end{equation}
for some constants $C_1,\gamma>0$.  This completes the argument that
\begin{equation}
  \bigl|\,
  \mathbb{E}\bigl[\hat{\sigma}_{\cp^a_s}^{(\mathrm{tr})}(V)\bigr]
  \;-\;
  \sigma_{\cp^a_s}(V)
  \bigr|
  \;\le\;
  C_1\,\|V\|\,
  e^{-\gamma\,N_{\max}}.
\end{equation}
Thus the bias decays \emph{exponentially} with $N_{\max}$.

\medskip
\textbf{Step~3: Bounded variance.}

Since $\hat{\sigma}_{\cp^a_s}(V)$ in \citep{wang2023model} has a variance uniformly bounded by $C_0\,\|V\|^2$, the truncated version is intuitively \emph{no larger}.  Formally, observe that:
\begin{itemize}
\item On $\{N<N_{\max}\}$, we have $N'=N$, so the truncated and untruncated estimators \emph{coincide}.
\item On $\{N\ge N_{\max}\}$, we have $N'=N_{\max}$, but $p'(N_{\max}) \ge p(N_{\max})$, meaning $\frac{1}{p'(N_{\max})}$ is \emph{no bigger} than $\frac{1}{p(N_{\max})}$.  Thus the magnitude of $\frac{\Delta_{N_{\max}}(V)}{p'(N_{\max})}$ is less than or comparable to that of $\frac{\Delta_{N}(V)}{p(N)}$ in the untruncated estimator.
\end{itemize}
Consequently,
\[
  \bigl\lvert
    \hat{\sigma}_{\cp^a_s}^{(\mathrm{tr})}(V)
  \bigr\rvert^2
  \;\;\le\;
  \mathrm{const}\,\bigl\lvert
     \hat{\sigma}_{\cp^a_s}(V)
  \bigr\rvert^2
  \quad
  \text{in all sample paths.}
\]
Taking expectations,
\[
  \mathbb{E}\Bigl[
     \bigl(\hat{\sigma}_{\cp^a_s}^{(\mathrm{tr})}(V)\bigr)^2
  \Bigr]
  \;\le\;
  \mathrm{const}\,\mathbb{E}\Bigl[
     \bigl(\hat{\sigma}_{\cp^a_s}(V)\bigr)^2
  \Bigr].
\]
By assumption,
\[
  \mathrm{Var}\bigl[\hat{\sigma}_{\cp^a_s}(V)\bigr]
  \;\le\;
  C_0\,\|V\|^2
  \quad\Longrightarrow\quad
  \mathbb{E}\Bigl[\bigl(\hat{\sigma}_{\cp^a_s}(V)\bigr)^2\Bigr]
  \;\le\;
  C'\,\|V\|^2
\]
for some $C'$.  Hence the truncated estimator has
\begin{equation}
  \mathrm{Var}\!\bigl[\hat{\sigma}_{\cp^a_s}^{(\mathrm{tr})}(V)\bigr]
  \;\le\;
  C_2\,\|V\|^2,
\end{equation}
where $C_2$ depends on $C'$ (and thus on $C_0$).  Thus its variance is uniformly bounded in $N_{\max}$.

\medskip
\textbf{Conclusion.}  
We have established that the truncated estimator $\hat{\sigma}_{\cp^a_s}^{(\mathrm{tr})}(V)$ has an exponentially decaying bias (as a function of $N_{\max}$) and a uniformly bounded variance.  This completes the proof.
\end{proof}

\begin{remark}
The same argument applies equally to the TV--distance setting, the KL--divergence setting, the $\chi^2$--distance setting, and the Wasserstein--distance setting (under discrete $\mcs$), because in each case:
\begin{enumerate}
\item The untruncated MLMC estimator is unbiased and has bounded variance \citep{wang2023model}.
\item The robust one--step operator $\sigma_{\cp^a_s}(V)$ is sufficiently continuous in the empirical distribution so that $\Delta_n(V)\to 0$ at a rate $\mathrm{O}(2^{-\,n/2})$.
\end{enumerate}
Hence the truncated version inherits the bounded variance property and gains only an exponentially small bias.
\end{remark}

\subsection{Robust Synchronous TD for Policy Evaluation}


\begin{algorithm}[ht]
\caption{Stochastic Robust Average-Reward TD Learning}
\label{alg:robust-avg-reward-TD}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Step-size sequence \(\{\alpha_t\}\), policy \(\pi\), and sampler from the nominal MDP (centroid of the uncertainty set).
\STATE \textbf{Initialize:} \(V_0(s) = 0 \;\;\forall s\in\mathcal{S},\quad g_0 = 0\)
\FOR{$t=0,1,2,\ldots,T-1$}
  \STATE \textbf{(a) Robust Bellman Approximation:}
    \begin{itemize}
      \item Sample a batch of states \(\{s^t_1,\dots,s^t_B\}\) (or collect all states if feasible).
      \item For each sampled \(s\), pick \(a\sim\pi(\cdot\mid s)\).
      \item Obtain estimates \(\widehat{\sigma}_t(s,a)\) of \(\sigma_{\mathcal{P}^a_s}(V_t)\)
            (e.g., via a minimization routine or a biased/unbiased estimator).
      \item Form the operator estimate:
            \[
               \widehat{T}_{g_t}V_t(s) \;=\; \sum_{a\in\mathcal{A}} \pi(a\mid s)\,
               \Bigl[\,
                   r(s,a) \;-\; g_t \;+\; \widehat{\sigma}_t(s,a)
               \Bigr].
            \]
    \end{itemize}
  \STATE \textbf{(b) Update Bias Function:}
    \[
       V_{t+1}(s)
       \;=\;
       V_t(s)
       \;+\;
       \alpha_t\,\Bigl(\widehat{T}_{g_t}V_t(s) \;-\; V_t(s)\Bigr),
       \quad \forall s\in \mathcal{S}.
    \]
    \STATE \quad (One may normalize \(V_{t+1}\) by subtracting \(V_{t+1}(s_0)\) from every component to anchor a reference state.)
  \STATE \textbf{(c) Update Average Reward:}
    \begin{itemize}
      \item Compute the residuals:
            \[
              \widehat{\delta}_t(s)
              \;=\;
              \sum_{a\in\mathcal{A}} \pi(a\mid s)\,r(s,a)
              \;+\;
              \sum_{a\in\mathcal{A}} \pi(a\mid s)\,\widehat{\sigma}_t(s,a)
              \;-\;
              V_t(s).
            \]
      \item Average the residuals:
            \[
               \overline{\delta}_t
               \;=\;
               \frac{1}{|\mathcal{S}|}\;\sum_{s\in\mathcal{S}}\;\widehat{\delta}_t(s).
            \]
      \item Update \(g\):
            \[
               g_{t+1}
               \;=\;
               g_t
               \;+\;
               \alpha_t\,\bigl(\,\overline{\delta}_t \;-\; g_t\bigr).
            \]
    \end{itemize}
\ENDFOR
\STATE \textbf{Output:} Final estimates \(\{V_T,\,g_T\}\).
\end{algorithmic}
\end{algorithm}

\noindent
\textbf{Description.} \\
The algorithm above provides a model-free policy evaluation method for robust average-reward Markov decision processes (MDPs). At iteration \(t\), it samples state--action pairs according to a fixed policy \(\pi\) on the nominal MDP. Using these samples, it obtains an approximate robust Bellman operator \(\widehat{T}_{g_t}V_t\) by estimating \(\sigma_{\mathcal{P}^a_s}(V_t)\), which is the worst-case expected bias term under the uncertainty set. The bias function \(V\) is then updated via a temporal-difference (TD) step with learning rate \(\alpha_t\). In parallel, the algorithm computes the residual \(\widehat{\delta}_t(s)\) and its average \(\overline{\delta}_t\), which measures how closely \(V\) aligns with the robust Bellman equation. The average reward parameter \(g\) is updated by moving it toward \(\overline{\delta}_t\). As \(t\) grows, both \(V_t\) and \(g_t\) converge to the fixed point of the robust average-reward Bellman equation, thus estimating the robust bias function and the robust average reward, respectively.

\begin{theorem}[Biased-Noise Variant of Theorem 3 with Sample Complexity]\label{thm:biasedNoiseExtended}
\emph{(cf.\ Theorem\,3 in \citep{zhang2021finite})}\,
Consider the stochastic approximation scheme
\begin{equation}\label{eq:updateRule}
  x^{t+1} \;=\; x^t \;+\; \eta_t \,\bigl[\,\widehat{H}(x^t) - x^t\bigr]\,,
  \quad t=0,1,2,\ldots,
\end{equation}
for finding an \emph{equivalent-class} fixed point \(x^*\in\mathbb{R}^n\) such that 
\[
  H(x^*) \;-\; x^* \;\in\;\overline{E},
  \quad \text{i.e. } \|H(x^*) - x^*\|_{c,\overline{E}} = 0.
\]
Here, \(\overline{E}\subseteq \mathbb{R}^n\) is a linear subspace, and we assume:

\begin{enumerate}
\item (\textbf{Contractive property in the semi-norm})
  For some \(\gamma\in(0,1)\),
  \[
    \|H(x) - H(y)\|_{c,\overline{E}}
    \;\le\;
    \gamma\,\|x - y\|_{c,\overline{E}}
    \quad\forall\,x,y\in \mathbb{R}^n.
  \]

\item (\textbf{Biased, bounded-variance noise}) For each iteration \(t\),
  \[
    \widehat{H}(x^t)
    \;=\;
    H(x^t)
    \;+\;
    w^t,
    \qquad
    \mathbb{E}[\,w^t \mid \mathcal{F}^t] 
    \;=\;
    \varepsilon_{\text{bias}}, 
    \qquad
    \mathbb{E}\bigl[\|\,w^t\|_{c,\overline{E}}^2 \,\big|\,
      \mathcal{F}^t\bigr]
    \;\le\;
    A 
    \;+\;
    B\,\|\,x^t - x^*\|_{c,\overline{E}}^2,
  \]
  for constants \(A,B \ge 0\) and a (possibly zero) bias vector \(\varepsilon_{\text{bias}}\).  
  The filtration \(\mathcal{F}^t\) is that generated by \(\{x^0,\ldots,x^t\}\).

\item (\textbf{Semi-Lyapunov function})
  Let \(M_{\overline{E}}(x)\) be defined by
  \[
    M_{\overline{E}}(x) 
    \;=\;
    \bigl(\,M \,\Box\, \delta_{\overline{E}}\bigr)(x),
  \]
  where \(M\) is a smooth, convex function used to ``regularize'' along the subspace \(\overline{E}\) (see \citep{zhang2021finite} for details). 
  By construction, there exist positive constants \(c_\ell,c_u\) such that
  \[
    c_\ell\,\|x - x^*\|_{c,\overline{E}}^2
    \;\le\;
    M_{\overline{E}}(x)
    \;\le\;
    c_u\,\|x - x^*\|_{c,\overline{E}}^2,
  \]
  and \(M_{\overline{E}}(\cdot)\) is \(L\)-smooth with respect to the semi-norm \(\|\cdot\|_{s,\overline{E}}\).  
\end{enumerate}

Then, under the step-size schedules:
\begin{itemize}
\item\textbf{(Decreasing step size)} 
  \(\displaystyle \eta_t \;=\;\frac{1}{\alpha_2\,(t+K)},\)
  with 
  \(\displaystyle K \;=\;\max\bigl\{\alpha_3/\alpha_2,\,3\bigr\}\),
\item\textbf{(Constant step size)} 
  \(\eta_t = \eta\) with \(\eta\,\alpha_3/\alpha_2 \le 1\),
\end{itemize}
the iteration \eqref{eq:updateRule} satisfies bounds analogous to those in \citep[Theorem\,3]{zhang2021finite}, but with additional bias-dependent terms. 
Specifically:

\begin{enumerate}
\item \emph{(Decreasing step size)} 
  \[
    \mathbb{E}\bigl[\|x^N - x^*\|_{c,\overline{E}}^2\bigr]
    ~\le~
    \frac{K^2}{(N+K)^2}\,\frac{c_u}{c_\ell}\,\|x^0 - x^*\|_{c,\overline{E}}^2
    \;+\;
    \frac{8\,\alpha_4\,c_u}{(N+K)\,\alpha_2^2}
    \;+\;
    \underbrace{\mathcal{O}\!\Bigl(\sum_{t=1}^N \eta_t\,\|\varepsilon_{\text{bias}}\|\Bigr)}_{\text{Bias term}}.
  \]
  In the special case \(\varepsilon_{\text{bias}}=0\), the bias term vanishes and this reduces exactly to \citep[Eq.\,(B.8)]{zhang2021finite}.

\item \emph{(Constant step size)} 
  \[
    \mathbb{E}\bigl[\|x^N - x^*\|_{c,\overline{E}}^2\bigr]
    ~\le~
    \bigl(1 - \alpha_2\bigr)^N \,\frac{c_u}{c_\ell}\,\|x^0 - x^*\|_{c,\overline{E}}^2
    \;+\;
    \frac{c_u\,\alpha_4}{\alpha_2}\,\eta
    \;+\;
    \underbrace{\mathcal{O}\!\bigl(\eta\,\|\varepsilon_{\text{bias}}\|\bigr)}_{\text{Bias term}}.
  \]
  Again, if \(\varepsilon_{\text{bias}}=0\), then we match \citep[Eq.\,(B.9)]{zhang2021finite} exactly.
\end{enumerate}

\paragraph{Sample complexity analysis.}
We now show how one obtains the typical \(\tilde{O}(\epsilon^{-2})\) complexity from these bounds.  For concreteness, consider the \emph{decreasing step-size} schedule, which yields 
\begin{align*}
\mathbb{E}\bigl[\|\,x^N - x^*\|_{c,\overline{E}}^2\bigr]
~\le~
\underbrace{\frac{K^2}{(N+K)^2}\,\frac{c_u}{c_\ell}\,\|x^0 - x^*\|_{c,\overline{E}}^2}_{\text{Term A}}
~+~
\underbrace{\frac{8\,\alpha_4\,c_u}{(N+K)\,\alpha_2^2}}_{\text{Term B}}
~+~
\underbrace{\mathcal{O}\!\Bigl(\sum_{t=1}^N \eta_t\,\|\varepsilon_{\text{bias}}\|\Bigr)}_{\text{Term C}}.
\end{align*}
We want this to be \(\le \epsilon^2\).  Observe that:
\begin{itemize}
\item \(\text{Term A} \approx \frac{1}{(N+K)^2}\) decays on the order of \(1/N^2\).
\item \(\text{Term B} \approx \frac{1}{N+K}\) decays on the order of \(1/N\).
\item \(\text{Term C} \approx \|\varepsilon_{\text{bias}}\|\sum_{t=1}^N \frac{1}{t+K}\) (since \(\eta_t = 1/[\alpha_2(t+K)]\)) grows roughly like \(\|\varepsilon_{\text{bias}}\|\ln N\).  
  - If \(\varepsilon_{\text{bias}}=0\), Term C disappears.  
  - If \(\varepsilon_{\text{bias}}\)\(\neq 0\) but small, we still get a mild \(\ln N\) factor.  
  - If \(\varepsilon_{\text{bias}}\) decays (e.g.\ exponentially in \(t\)), then Term C remains uniformly bounded.
\end{itemize}

\noindent
Hence, for \(\varepsilon_{\text{bias}} = 0\) (no bias), balancing Term B with \(\epsilon^2\) suggests:
\[
  \frac{1}{N} \;=\; O(\epsilon^2)
  \quad\Rightarrow\quad 
  N \;=\;O\bigl(\tfrac{1}{\epsilon^2}\bigr).
\]
Thus the sample/iteration complexity (the number of steps required so that the left-hand side is \(O(\epsilon^2)\)) is \(O(\epsilon^{-2})\).  

\smallskip

\noindent
\textbf{Case with bias:}
\begin{itemize}
\item If \(\varepsilon_{\text{bias}}\neq 0\) is constant, you converge only to a bias-dependent neighborhood of \(x^*\).  In that case, you cannot drive the error below a constant times \(\|\varepsilon_{\text{bias}}\|\).  

\item If \(\varepsilon_{\text{bias}}\) itself decays (e.g.\ exponentially) to zero, then for large \(t\), \(\|\varepsilon_{\text{bias}}\|\) is negligible, and \emph{effectively} we recover the same \(O(\epsilon^{-2})\) complexity for driving the residual below \(\epsilon\). 
\end{itemize}
A similar argument applies under the \emph{constant step size} scenario, but there the final bound has a geometric decay plus a constant ``variance'' offset, plus a bias offset.  The net result is also that you can achieve an \(\epsilon\)-level accuracy in \(O(\log(1/\epsilon))\) steps if ignoring variance, or remain in an \(\varepsilon_{\text{bias}}\)-proportional ball.

\end{theorem}

\begin{proof}[Proof Sketch]
See \citep{zhang2021finite} for the case of zero-mean martingale noise; the difference here is that 
\(\mathbb{E}[\,w^t \mid \mathcal{F}^t] \;=\;\varepsilon_{\text{bias}}\neq 0\).  
This introduces an extra term \(\eta_t \langle \nabla M_{\overline{E}}(x^t),\varepsilon_{\text{bias}}\rangle\) in the standard one-step analysis.  As in \citep[Lem.\,5]{zhang2021finite}, we combine the $L$-smoothness of \(M_{\overline{E}}\) and the $\gamma$-contractive property of \(H\) to show a negative drift in $M_{\overline{E}}(x^t-x^*)$ except for the noise terms.  The variance-boundedness yields a $\eta_t^2$ term, while the bias yields a $\eta_t$ term multiplied by $\|\varepsilon_{\text{bias}}\|$.  Summing or telescoping over $t=0$ to $N-1$ then yields the above recursion.  Finally, choosing $\eta_t=1/[\alpha_2(t+K)]$ (or $\eta_t=\eta$ constant) completes the derivation of the explicit bounds \citep[see also Eq.\,(B.8)--(B.9)]{zhang2021finite}.
\end{proof}



\begin{theorem}[Stochastic Approximation with Mini-batches and Decaying Bias]
\label{thm:MiniBatchDecayingBias}
Suppose we run the stochastic approximation update
\begin{equation}\label{eq:MiniBatchUpdate}
  x^{t+1} \;=\; x^t \;+\; \eta_t \bigl[\widehat{H}(x^t) - x^t\bigr],
\end{equation}
aiming to solve a contraction in the semi-norm
\(\|\!\cdot\!\|_{c,\overline{E}}\) (as in 
\citep[Assumption\,4]{zhang2021finite}
or Theorem\,\ref{thm:biasedNoiseExtended} above).
The difference here is:
\begin{enumerate}
\item \textbf{Mini-batch sampling.} 
  Each iteration \(t\) uses a mini-batch of size on the order of
  \(\log(N_{\max})\) 
  to estimate \(H(x^t)\).  Thus, if we run \(N\) total iterations, the \emph{total} sample usage is
  \(\widetilde{O}(N) \;=\; O\bigl(N \,\log(N_{\max})\bigr)\).
\item \textbf{Polynomially decaying bias.}
  The noise term \(w^t\) has expectation
  \(\mathbb{E}[w^t\mid\mathcal{F}^t] 
    = \varepsilon_{\text{bias}}^{\,t},\)
  where
  \(\|\varepsilon_{\text{bias}}^{\,t}\|\;=\;O\bigl(t^{-p}\bigr)\)
  for some \(p>0\).
  In particular, a common example is \(p=\tfrac12\) so that
  \(\|\varepsilon_{\text{bias}}^{\,t}\| = O\bigl(t^{-1/2}\bigr)\).
\item \textbf{Bounded (or mild) variance.} 
  We retain the usual assumption:
  \[
    \mathbb{E}\bigl[\|\,w^t\|_{c,\overline{E}}^2 
      \,\big|\,
      \mathcal{F}^t\bigr]
    \;\le\;
    A \;+\; B\,\|x^t - x^*\|_{c,\overline{E}}^2
    \quad\text{for constants }A,B\!\ge0.
  \]
\end{enumerate}
Then, under the same step-size choices (decreasing or constant) as in 
\citep[Theorem\,3]{zhang2021finite}
and Theorem\,\ref{thm:biasedNoiseExtended}, we achieve the usual 
\(\epsilon^{-2}\) \emph{iteration} complexity in order to make
\(\mathbb{E}[\|x^N-x^*\|_{c,\overline{E}}^2]\le \epsilon^2\).  
\emph{Moreover,} each iteration uses 
\(O(\log(N_{\max}))\) samples, so the \textbf{total sample complexity} is
\[
  \widetilde{O}\bigl(\epsilon^{-2}\bigr)
  \quad
  \text{(suppressing logarithmic factors).}
\]

\end{theorem}

\begin{proof}[Proof Sketch]
We outline the three main points:

\paragraph{1. Mini-batch with log-factors.}
Because each iteration uses a mini-batch of size proportional to \(\log(N_{\max})\), the variance of the noise estimate \(\widehat{H}(x^t)\) can be reduced by approximately a factor of \(\log(N_{\max})\).  Concretely, if each \(\widehat{H}(x^t)\) is formed by averaging \(\Theta(\log(N_{\max}))\) i.i.d.\ samples, then the variance satisfies
\[
   \mathbb{E}\bigl[\|w^t\|^2_{c,\overline{E}}\bigr]
   \;=\;
   O\!\Bigl(\tfrac{1}{\log(N_{\max})}\Bigr)
   \quad
   \text{(if originally on the order of 1).}
\]
All the classical SA bounds in \citep{zhang2021finite} (and references therein) then apply with this effectively smaller variance.

\paragraph{2. Polynomially decaying bias.}
We now have
\(\mathbb{E}[w^t \mid \mathcal{F}^t] 
   = \varepsilon_{\text{bias}}^{\,t}\),
with \(\|\varepsilon_{\text{bias}}^{\,t}\| = O(t^{-p})\).  
When unrolling the usual Lyapunov or smoothness argument, the bias contributes an extra term of the form
\[
   \sum_{t=1}^N \eta_t\,\bigl\|\varepsilon_{\text{bias}}^{\,t}\bigr\|.
\]
Assuming a decreasing step size \(\eta_t \approx 1/t\), 
we get a sum like
\[
   \sum_{t=1}^N 
     \frac{1}{t}\cdot \frac{1}{t^p}
   \;=\;
   \sum_{t=1}^N
     \frac{1}{t^{\,1+p}},
\]
which is finite (convergent) for \(p>0\).  Hence the bias term does \emph{not} accumulate unboundedly and does not degrade the overall \(1/N\)- or \(1/\sqrt{N}\)-style rates typically seen in SA.  

\paragraph{3. Net effect on sample complexity.}
Let \(N\) be the total number of outer iterations.  From Theorem\,\ref{thm:biasedNoiseExtended} (or \citep[Theorem\,3]{zhang2021finite}), we know the iteration count \(N\) needed to satisfy 
\(\mathbb{E}[\|x^N - x^*\|^2_{c,\overline{E}}]\le \epsilon^2\)
scales on the order of \(\epsilon^{-2}\).  
But each iteration now uses \(\Theta(\log(N_{\max}))\) samples.  If we take \(N_{\max} \approx N\approx \epsilon^{-2}\), then each iteration uses about \(\log(1/\epsilon)\) samples.  Hence the \emph{total sample usage} is
\[
   N \,\times\, O(\log(N_{\max}))
   \;\approx\;
   O\Bigl(\tfrac{1}{\epsilon^2}\,\log(\tfrac{1}{\epsilon})\Bigr),
\]
which is denoted 
\(\widetilde{O}\bigl(\epsilon^{-2}\bigr)\) 
by suppressing constant and polylogarithmic factors.  

Combining these points shows that mini-batching with a mild (logarithmic) cost per iteration plus a polynomially decaying bias still yields an \(\epsilon^{-2}\) iteration complexity, and thus an overall sample complexity of \(\widetilde{O}(\epsilon^{-2})\).
\end{proof}



\begin{theorem}[Finite-Sample Bound for the Average-Reward Parameter]
\label{thm:avg-reward-bound}
Consider the update
\[
  g_{t+1}
  \;=\;
  g_t
  \;+\;
  \alpha_t\bigl[\overline{\delta}_t - g_t\bigr],
  \quad
  \overline{\delta}_t
  \;=\;
  \delta(V_t)
  \;+\;
  W_t,
\]
where $g^*$ is the true robust average reward satisfying
\(\,\delta(V^*)=g^*\), and $W_t$ is a (possibly biased) noise process with
\(\mathbb{E}[|W_t|\mid \mathcal{F}_t]=\epsilon_{\mathrm{bias}}\) and bounded variance.
Then for any $N\ge1$ and suitable step sizes $\{\alpha_t\}$, the iterates $g_N$ satisfy:
\[
  \mathbb{E}\bigl[\,(g_N - g^*)^2\bigr]
  \;\;\le\;\;
  C_1\,\epsilon_{\mathrm{bias}}^2
  \;+\;
  C_2\,\mathbb{E}\!\Bigl[\bigl\|x^N - x^*\bigr\|_{\mathrm{span}}^2\Bigr]
  \;+\;
  \text{(terms that vanish under a standard SA schedule).}
\]
Here $x^N$ is the joint state of the $(V,g)$ iterates, and $C_1,C_2$ are positive constants
depending on the MDP parameters and the noise bounds.
\end{theorem}

\begin{proof}
Let $e_t \;\triangleq\; g_t - g^*$, and define a scalar Lyapunov function
\[
  M_g(e) \;=\; \tfrac12\,(e)^2.
\]
Using the Bellman-residual decomposition
\(\,\overline{\delta}_t = \delta(V_t) + W_t,\)
we rewrite the update for $g_{t+1}$ in terms of $e_t$:
\[
  e_{t+1}
  \;=\;
  e_t
  \;+\;
  \alpha_t \Bigl[\delta(V_t) - g^* + W_t - e_t\Bigr]
  \;=\;
  e_t + \alpha_t\bigl[\Delta_t^{(g)} + W_t - e_t\bigr],
\]
where
\(\,\Delta_t^{(g)} \;\triangleq\; \delta(V_t) - g^*.\)

\noindent
\textbf{Step 1: Expand the Lyapunov.}
\[
  M_g\bigl(e_{t+1}\bigr)
  \;=\;
  \tfrac12\,(e_{t+1})^2
  \;=\;
  \tfrac12\,
   \bigl[e_t + \alpha_t(\Delta_t^{(g)} + W_t - e_t)\bigr]^2.
\]
A straightforward expansion yields
\[
  M_g(e_{t+1})
  \;=\;
  M_g(e_t)
  \;+\;
  \alpha_t\,e_t\,\Delta_t^{(g)}
  \;+\;
  \alpha_t\,e_t\,W_t
  \;-\;
  \alpha_t\,(e_t)^2
  \;+\;
  \tfrac12\,\alpha_t^2
     \bigl[\Delta_t^{(g)} + W_t - e_t\bigr]^2.
\]

\noindent
\textbf{Step 2: Take conditional expectation.}
Denote by $\mathcal{F}_t$ the sigma-algebra up to time $t$. We know:
\[
  \mathbb{E}[\,|W_t|\mid \mathcal{F}_t] \;=\; \epsilon_{\mathrm{bias}},
  \quad
  \mathbb{E}\bigl[\,|W_t|^2 \mid \mathcal{F}_t\bigr]\;\le\;\sigma^2,
\]
and $\Delta_t^{(g)}$ depends only on $V_t$ (hence is $\mathcal{F}_t$-measurable).
Applying $\mathbb{E}[\cdot\mid \mathcal{F}_t]$ to each term gives
\[
  \mathbb{E}\bigl[M_g(e_{t+1})\bigr]
  \;\le\;
  \mathbb{E}\bigl[M_g(e_t)\bigr]
  \;-\;
  \alpha_t\,\mathbb{E}\bigl[(e_t)^2\bigr]
  \;+\;
  \alpha_t\,\mathbb{E}[\,e_t\,\Delta_t^{(g)}\,]
  \;+\;
  \alpha_t\,\epsilon_{\mathrm{bias}}
      \,\mathbb{E}\bigl[|e_t|\bigr]
  \;+\;
  \mathcal{O}\bigl(\alpha_t^2\bigr),
\]
where the $\mathcal{O}(\alpha_t^2)$ term includes
$\alpha_t^2\,\sigma^2$ and similar bounded-variance contributions.

\noindent
\textbf{Step 3: Summation and telescoping.}
Summing over $t=0$ to $N-1$, we telescope
\[
  \mathbb{E}[\,M_g(e_N)\,]
  \;=\;
  \mathbb{E}\bigl[\tfrac12\,(g_N-g^*)^2\bigr]
  \;\le\;
  \bigl[\text{(initial terms)}\bigr]
  \;+\;
  \sum_{t=0}^{N-1}
   \Bigl(\,\alpha_t\,\epsilon_{\mathrm{bias}}\,\mathbb{E}[\,|e_t|\,]
     \;+\;
     \alpha_t\,\mathbb{E}[\,e_t\,\Delta_t^{(g)}\,]
     \;+\;
     \alpha_t^2\,\sigma^2
   \Bigr)
   \;-\;
   \sum_{t=0}^{N-1}
   \alpha_t\,\mathbb{E}[(e_t)^2].
\]
We further note that $\Delta_t^{(g)} = \delta(V_t)-g^*$ is bounded by
some constant times $\|V_t - V^*\|_{\mathrm{span}}$, and
$\sum_{t}\alpha_t^2$ is typically finite for a standard SA schedule
(e.g.\ $\alpha_t=\alpha_0/t$).
Hence, collecting these terms yields a bound of the form
\[
  \mathbb{E}\bigl[(g_N - g^*)^2\bigr]
  \;\le\;
  C_1\,\epsilon_{\mathrm{bias}}^2
  \;+\;
  C_2\,\mathbb{E}\bigl[\|x^N - x^*\|_{\mathrm{span}}^2\bigr]
  \;+\;
  \text{other terms that vanish as }N\to\infty
  \text{ under suitable }\{\alpha_t\}.
\]
Therefore, $g_N$ converges up to an offset controlled by the bias level
$\epsilon_{\mathrm{bias}}$ and the accuracy of $V_t$, completing the proof.
\end{proof}

